Measurement of the charge asymmetry in dileptonic decays of top quark pairs in proton-proton collisions at 7 TeV using the ATLAS detector

A measurement of the top--antitop ($t\bar{t}$) charge asymmetry is presented using 2011 LHC data collected by the ATLAS detector corresponding to an integrated luminosity of 4.6 fb$^{-1}$ at a centre-of-mass energy of 7 TeV. The analysis is performed in the dilepton channel, and two different observables are studied: $A^{\ell\ell}_{\mathrm{C}}$, based on the identified charged leptons, and $A^{t\bar{t}}_{\mathrm{C}}$, based on the reconstructed $t\bar{t}$ final state. The asymmetries, measured to be $A^{\ell\ell}_{\mathrm{C}} = 0.024 \pm 0.015 \mathrm{(stat.)} \pm 0.009 \mathrm{(syst.)}$ and $A^{t\bar{t}}_{\mathrm{C}} = 0.021 \pm 0.025 \mathrm{(stat.)} \pm 0.017 \mathrm{(syst.)}$, are in agreement with the Standard Model predictions.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = proceedings

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	$(BIBTEX) ${BASENAME}
	$(BIBTEX) ${BASENAME}
	pdflatex  ${BASENAME}
	$(BIBTEX) ${BASENAME}
	$(BIBTEX) ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg \
              *.inx *.dvi *.toc *.out *~ ~* */*~ */~* spellTmp 

